Rotation Equivariant Siamese Networks for Tracking

Rotation is among the long prevailing, yet still unresolved, hard challenges encountered in visual object tracking. The existing deep learning-based tracking algorithms use regular CNNs that are inherently translation equivariant, but not designed to tackle rotations. In this paper, we first demonstrate that in the presence of rotation instances in videos, the performance of existing trackers is severely affected. To circumvent the adverse effect of rotations, we present rotation-equivariant Siamese networks (RE-SiamNets), built through the use of group-equivariant convolutional layers comprising steerable filters. SiamNets allow estimating the change in orientation of the object in an unsupervised manner, thereby facilitating its use in relative 2D pose estimation as well. We further show that this change in orientation can be used to impose an additional motion constraint in Siamese tracking through imposing restriction on the change in orientation between two consecutive frames. For benchmarking, we present Rotation Tracking Benchmark (RTB), a dataset comprising a set of videos with rotation instances. Through experiments on two popular Siamese architectures, we show that RE-SiamNets handle the problem of rotation very well and out-perform their regular counterparts. Further, RE-SiamNets can accurately estimate the relative change in pose of the target in an unsupervised fashion, namely the in-plane rotation the target has sustained with respect to the reference frame.

==> baselines.tex <==
% \textbf{Base Siamese trackers. }For benchmarking the results of tracking, the most suitable baselines would be the base Siamese trackers that are being adapted. In this paper, we conduct most experiments with respect to SiamFC \cite{bertinetto2016fully}, and its architectural variant SiamFCv2. These two are chosen as baselines for validating most results of this paper. Further, we perform a preliminary experiment on adding rotation equivariance in SiamRPN++ \cite{li2019siamrpn++}, and in this case, SiamRPN++ is the baseline. 

% \textbf{Other baselines. }For comparing tracking performance, other baselines include the two variants of DiMP \cite{bhat2019learning}, one of the SOTA methods. Since no previous works exist on 2D orientation estimation in an unsupervised manner, we benchmark these results using the majority baselines as well as in terms of variance reduction in the case of regression formulation. To evaluate the advantage of imposing constraint on rotational motion, we compare the scenarios of tracking with and without this constraint.


==> data.tex <==
\textbf{Training. }All rotation equivariant variants of SiamFC are trained on the GOT-10k \cite{huang2019got} training set. To train SiamRPN++, we trained a rotation equivariant version of ResNet50 architecture on ImageNet. The SiamRPN++ model was then trained using this backbone on sets of COCO \cite{}, ImageNet DET \cite{}, ImageNet VID \cite{} and YouTube-BoundingBoxes \cite{} datasets.

\textbf{Evaluation. }The RE-SiamNets developed in this work are evaluated on various datasets. To evaluate how well these perform in presence of frequent in-plane rotations, we test them on ROB35, rot-OTB100 and rot-MNIST datasets. To demonstrate that adding RE-SiamNets do not degrade the performance of trackers with respect to other challenges, we test them on some common tracking benchmarks that include OTB100 \cite{}, GOT-10k \cite{} and LaSOT \cite{}. 

==> pgfplots/app_schematic.tex <==
\begin{figure*}
\begin{minipage}{1\textwidth}
    \centering
    % \begin{subfigure}{1.0\textwidth}
    % \centering
    % \includegraphics[scale=0.35]{images/schematics/Rot_siam_fig2a_fin-2.pdf}
    % \end{subfigure}
    \begin{subfigure}{1.0\textwidth}
    \centering
    \begin{tikzpicture}
    \draw (0, 0) node[inner sep=0] {\fbox{\includegraphics[scale=0.5]{images/schematics/same_fig.pdf}}};
    \draw(-3.7,1) node {$x$};
    \draw(-4.75,2.9) node {\rotatebox{48}{{\scriptsize$z_1, z_2,.., z_{\Lambda}$}}};
    \draw(-3.3,2) node {$Z$};
    \draw(-2.6,2.67) node {$\phi$};
    \draw(-2.6,0.5) node {$\phi$};
    \draw(-1.4,-0.2) node {$\phi(x)$};
    \draw(-1.4,3.1) node {{\small$\{\phi(z)\}$}};
    \draw(2.5,0.3) node {{\small$\{\hat{h}(z,x)\}$}};
    \draw(4.8,0.7) node {{\small$h(z,x)$}};
    \draw(-2.5,1.6) node {{\footnotesize RE-encoding}};
    \draw(0.91,1.97) node {$*$};
    \draw(0.34,1.38) node {$*$};
    \draw(-0.07,1.0) node {$*$};
    %\draw(-0.2,2.1) node {{\footnotesize $\mathcal{R}_{{\theta}_1}$}};
    %\draw(0.37,2.5) node {{\footnotesize $\mathcal{R}_{{\theta}_2}$}};
    %\draw(0.77,3.2) node {{\footnotesize $\mathcal{R}_{{\theta}_{\Lambda}}$}};
    \draw(3.8,1.45) node {{\scriptsize Global}};
    \draw(3.8,1.15) node {{\scriptsize maxpooling}};
    \draw(3.50,-0.1) node {{\small $Z$ - template set}};
    \draw(3.8,-0.4) node {{\small $x$ - candidate frame}};
    
    \draw(-1.55,-1.67) node {{\small $*$}};
    \draw(-1.55,-2.16) node {{\small $*$}};
    \draw(-1.55,-2.48) node {{\small $*$}};
    \draw(-4.37,-2.0) node {{\small $*$}};
    
    \draw(5,3) node {(a)};
    \draw(5,-1.1) node {(b)};
    
    %\draw(-4.08,-2.25) node {{\scriptsize $\Psi$}};
    %\draw(-3.69,-2.0) node {{\scriptsize \rotatebox{45}{$\Psi$}}};
    %\draw(-3.27,-1.72) node {{\scriptsize \rotatebox{90}{$\Psi$}}};
    \end{tikzpicture}
    \end{subfigure}
    \caption{(a) Schematic representation of RE-SiamNet typically designed for object tracking. On the template head, $\Lambda$ equidistant rotated variants of the original template image are used. (b) Basic structure of the steerable CNN based on  \protect\cite{weiler2018learning} for rotation-equivariant image to feature-map translation. For clarity, only a single group-convolution layer is shown, and the rest is omitted. As shown, applying a rotation of 90 degrees, $\rho_{90}$, on the input image produces feature map rotated by the same amount.}
    \label{app_img_resiam}
\end{minipage}
\begin{minipage}{1\textwidth}
%\setlength{\fboxsep}{0.5pt}
\frame{
\begin{subfigure}{1.0\textwidth}
    \centering
    \includegraphics[height=1.67cm, width=2.8cm]{images/annotation/pig1.pdf}
    \includegraphics[width=2.8cm, height=1.67cm]{images/annotation/pig2.pdf}
    \includegraphics[height=1.67cm, width=2.8cm]{images/annotation/pig1.pdf}
    \includegraphics[width=2.8cm, height=1.67cm]{images/annotation/pig1.pdf}
    \includegraphics[height=1.67cm, width=2.8cm]{images/annotation/pig1.pdf}
    \includegraphics[width=2.8cm, height=1.67cm]{images/annotation/pig1.pdf}
    \includegraphics[height=1.67cm, width=2.8cm]{images/annotation/pig1.pdf}
\includegraphics[width=2.8cm, height=1.67cm]{images/annotation/pig1.pdf}
    \includegraphics[height=1.67cm, width=2.8cm]{images/annotation/pig1.pdf}
\includegraphics[width=2.8cm, height=1.67cm]{images/annotation/pig1.pdf}
\end{subfigure}}
    \caption{Example frames from 4 sequences of ROB dataset with annotations for target location and orientation.}
    \label{fig_rob_samples}
\end{minipage}
\end{figure*}

==> results.tex <==
% \subsection{Rotation Equivariance in Tracking}
% \input{tracking-results}

% \input{pose-results}

% \input{motion_cons}

==> train_eval.tex <==
\textbf{Training. }To train all the RE-SiamNet equivalents of SiamFC \cite{bertinetto2016fully}, we use the GOT-10k training set \cite{huang2019got}.

For the RE-SiamRPN implementations, we adapt the existing architecture of SiamRPN++, and train the model on  

\textbf{Evaluation. }sdfs



